Interpretable hypothesis tests

Although hypothesis tests play a prominent role in Science, their interpretation can be challenging. Three issues are (i) the difficulty in making an assertive decision based on the output of an hypothesis test, (ii) the logical contradictions that occur in multiple hypothesis testing, and (iii) the possible lack of practical importance when rejecting a precise hypothesis. These issues can be addressed through the use of agnostic tests and pragmatic hypotheses.

==> proofs.tex <==
\appendix

\section{Proofs}
\label{sec:proof}



